Evil from Within: Machine Learning Backdoors through Hardware Trojans

Backdoors pose a serious threat to machine learning, as they can compromise the integrity of security-critical systems, such as self-driving cars. While different defenses have been proposed to address this threat, they all rely on the assumption that the hardware on which the learning models are executed during inference is trusted. In this paper, we challenge this assumption and introduce a backdoor attack that completely resides within a common hardware accelerator for machine learning. Outside of the accelerator, neither the learning model nor the software is manipulated, so that current defenses fail. To make this attack practical, we overcome two challenges: First, as memory on a hardware accelerator is severely limited, we introduce the concept of a minimal backdoor that deviates as little as possible from the original model and is activated by replacing a few model parameters only. Second, we develop a configurable hardware trojan that can be provisioned with the backdoor and performs a replacement only when the specific target model is processed. We demonstrate the practical feasibility of our attack by implanting our hardware trojan into the Xilinx Vitis AI DPU, a commercial machine-learning accelerator. We configure the trojan with a minimal backdoor for a traffic-sign recognition system. The backdoor replaces only 30 (0.069%) model parameters, yet it reliably manipulates the recognition once the input contains a backdoor trigger. Our attack expands the hardware circuit of the accelerator by 0.24% and induces no run-time overhead, rendering a detection hardly possible. Given the complex and highly distributed manufacturing process of current hardware, our work points to a new threat in machine learning that is inaccessible to current security mechanisms and calls for hardware to be manufactured only in fully trusted environments.

==> figures/hw-trojan/eval-plot.tex <==
\definecolor{blue}{rgb}{0.12, 0.56, 1.0}
\definecolor{red}{rgb}{1.0, 0.0, 0.0}
\definecolor{yellow}{rgb}{1.0, 0.65, 0.0}
\definecolor{black}{rgb}{0.0,0.0,0.0}
\definecolor{green}{rgb}{0.196, 0.659, 0.321}

\begin{tikzpicture}


\begin{axis}[
      title = {},
      %legend style = {legend to name = grouplegend,},
      xlabel={number of replaced parameters},
      ylabel style={align=center},
      ylabel={success rate\\and test\\accuracy (\%)},
      axis on top,
      grid style={on layer=axis background},
      label style={font=\small},
      ymin=25, ymax=100,
      ytick={25,50,75,100},
      legend style = {column sep = 3pt, legend columns = 1, font=\footnotesize},
      tick label style={font=\small},
      legend cell align={left},
      legend pos=south east,
      enlarge x limits=0,
      enlarge y limits=0,
      width = 0.6\linewidth,
      height = 3.2cm,
      grid = both
    ]


\addplot[color=black, line width=0.3mm] plot [] table [x=name, y=success-rate, col sep=comma]{data/hw-trojan/evaluation-casestudy.csv};
\addlegendentry{success rate}

\addplot[color=black, line width=0.3mm, dashed] plot [] table [x=name, y=accuracy, col sep=comma]{data/hw-trojan/evaluation-casestudy.csv};
\addlegendentry{test accuracy}


\end{axis}
\end{tikzpicture}

==> figures/hw-trojan/overhead-plot.tex <==
\definecolor{blue}{rgb}{0.12, 0.56, 1.0}
\definecolor{red}{rgb}{1.0, 0.0, 0.0}
\definecolor{yellow}{rgb}{1.0, 0.65, 0.0}
\definecolor{black}{rgb}{0.0,0.0,0.0}
\definecolor{green}{rgb}{0.196, 0.659, 0.321}

\begin{tikzpicture}


\begin{axis}[
      title = {},
      %legend style = {legend to name = grouplegend,},
      xlabel={\# replaced parameters},
      ylabel style={align=center},
      ylabel={hardware\\overhead (\%)},
      axis on top,
      grid style={on layer=axis background},
      label style={font=\small},
      ymin=0, ymax=1.5,
      %ytick={1,10,100, 1000},
      legend style = {column sep = 3pt, legend columns = 1, font=\footnotesize},
      tick label style={font=\small},
      legend cell align={left},
      legend pos=north west,
      enlarge x limits=0,
      enlarge y limits=0,
      width = 0.6\linewidth,
      height = 4cm,
      grid = both
    ]


\addplot[color=black, line width=0.3mm] plot [] table [x=name, y=lut, col sep=comma]{data/hw-trojan/overhead-casestudy.csv};
\addlegendentry{LUTs}

\addplot[color=black, line width=0.3mm, dashed] plot [] table [x=name, y=ff, col sep=comma]{data/hw-trojan/overhead-casestudy.csv};
\addlegendentry{FFs}

\addplot[color=black, line width=0.3mm, dotted] plot [] table [x=name, y=lutram, col sep=comma]{data/hw-trojan/overhead-casestudy.csv};
\addlegendentry{LUT-RAM}


\end{axis}
\end{tikzpicture}

==> figures/ml-trojan/norm-plot.tex <==
% \definecolor{col1}{rgb}{0.12, 0.56, 1.0}
% \definecolor{col2}{rgb}{1.0, 0.0, 0.0}
% \definecolor{col3}{rgb}{1.0, 0.65, 0.0}
% \definecolor{col4}{rgb}{0.0,0.0,0.0}
% \definecolor{col5}{rgb}{0.196, 0.659, 0.321}

% \definecolor{col1}{HTML}{648FFF}
% \definecolor{col2}{HTML}{785EF0}
% \definecolor{col3}{HTML}{DC267F}
% \definecolor{col4}{HTML}{FE6100}
% \definecolor{col5}{HTML}{FFB000}

\definecolor{col1}{HTML}{332288}
\definecolor{col2}{HTML}{117733}
\definecolor{col3}{HTML}{88CCEE}
\definecolor{col4}{HTML}{DDCC77}
\definecolor{col5}{HTML}{882255}

\begin{tikzpicture}
\begin{groupplot}[group style = {group size = 3 by 1,
    horizontal sep = 50pt,
    vertical sep=20pt},
    %tick label style={font=\small},
    width = 0.33\linewidth,
    height = 0.33\linewidth
]

\nextgroupplot [
      title = {},
      %legend style = {legend columns = 1, text = black, at={(0.7,0.95)}, font=\footnotesize},
      xlabel={$\delta$},
      ylabel={$\lVert\delta\rVert_0$},
      axis on top,
      grid style={on layer=axis background},
      tick label style={font=\small},
      label style={font=\small},
      xtick={-2,0,2},
      ytick={0,2,4},
      ymin=0, ymax=4,
      %ytick={1,10,100, 1000},
      % enlarge x limits=0.02,
      % enlarge y limits=0.02,
      enlarge x limits=0,
      enlarge y limits=0,
      grid=both
    ]
    \addplot[domain=-2:-0.01, samples=2, color=col1, line width=0.3mm, forget plot]{1};
    \addplot[domain=0.01:2, samples=2, color=col1, line width=0.3mm, forget plot]{1};
    \addplot[domain=-0.01:0.0, samples=100, color=col1, line width=0.3mm, forget plot]{-100*x};
    \addplot[domain=0:0.01, samples=100, color=col1, line width=0.3mm]{100*x};
    %\addlegendentry{$p=0$}

    \nextgroupplot [
      title = {},
      %legend style = {legend columns = 1, text = black, at={(0.7,0.95)}, font=\footnotesize},
      xlabel={$\delta$},
      ylabel={$\lVert\delta\rVert_1$},
      axis on top,
      grid style={on layer=axis background},
      tick label style={font=\small},
      label style={font=\small},
      xtick={-2,0,2},
      ytick={0,2,4},
      ymin=0, ymax=4,
      %ytick={1,10,100, 1000},
      % enlarge x limits=0.02,
      % enlarge y limits=0.02,
      enlarge x limits=0,
      enlarge y limits=0,
      grid=both
    ]
    \addplot[domain=-2:0, samples=2, color=col2, line width=0.3mm, forget plot]{-x};
    \addplot[domain=0:2, samples=2, color=col2, line width=0.3mm]{x};
    %\addlegendentry{$p=1$}

    \nextgroupplot [
      title = {},
      %legend style = {legend columns = 1, text = black, at={(0.7,0.95)}, font=\footnotesize},
      xlabel={$\delta$},
      ylabel={$\lVert\delta\rVert^2_2$},
      axis on top,
      grid style={on layer=axis background},
      tick label style={font=\small},
      label style={font=\small},
      xtick={-2,0,2},
      ytick={0,2,4},
      ymin=0, ymax=4,
      %ytick={1,10,100, 1000},
      % enlarge x limits=0.02,
      % enlarge y limits=0.02,
      enlarge x limits=0,
      enlarge y limits=0,
      grid=both
    ]
    \addplot[domain=-2:2, samples=100, color=col5, line width=0.3mm]{x*x};
    %\addlegendentry{$p=2$}
    % \addplot[domain=-2:2, samples=3, color=black]{0};
    
\end{groupplot}
\end{tikzpicture}

==> sections/03_related_work.tex <==
\section{Related Work}
\label{dpu_trojan:subsec::discussion::related_work}

\par\smallskip\textbf{Fault Injection Attacks}
TODO: Talk about\cite{DBLP:conf/ccs/BreierHJMB018,DBLP:conf/iccad/LiuWLX17,DBLP:conf/iccv/RakinHF19,DBLP:conf/iclr/BaiWZL0X21,DBLP:conf/cvpr/RakinHF20,DBLP:conf/uss/HongFKGD19,DBLP:conf/uss/YaoRF20,DBLP:conf/dsn/TolIASZ23}


The rising popularity of neural networks also raised interest in backdoor attacks. 
Gu~\etal~\cite{DBLP:journals/access/GuLDG19} showed that an attacker can implant a backdoor by injecting malicious samples to the training dataset.
In contrast, our attack does not require any access to training data.
Tang~\etal~\cite{DBLP:conf/kdd/TangDLYH20} assume that an attacker can insert additional neuron connections, also resulting in a stronger attacker model than ours.
Further approaches relax the assumption of access to the training data~\cite{DBLP:conf/ndss/LiuMALZW018}, the visibility and position of the trigger~\cite{DBLP:journals/corr/abs-1712-05526,DBLP:conf/aaai/SahaSP20,DBLP:conf/nips/NguyenT20}, or the number of malicious examples required~\cite{DBLP:conf/nips/ShafahiHNSSDG18}. 
In terms of minimal changes, Rakin \etal~\cite{DBLP:conf/cvpr/RakinHF20} propose a backdoor that minimizes the required bit flips, but can lead to a drop in test accuracy of
up to 15\%.
Stealthy backdoors that are inserted during model compilation~\cite{DBLP:conf/satml/CliffordSZAM24}, model quantization~\cite{DBLP:journals/tdsc/MaQGZAXFZAA24}, or implemented by the software execution environment~\cite{DBLP:conf/icse/LiH0CL21} were also proposed recently.

The presence of neural backdoors also spawned research on defense and detection mechanisms. 
One line of research tries to detect directly whether a trigger is present in the model, for example by finding shortcuts between output classes~\cite{DBLP:conf/sp/WangYSLVZZ19}, training meta models to classify networks~\cite{DBLP:conf/sp/XuWLBGL21}, or utilizing statistical properties from model predictions~\cite{DBLP:conf/ijcai/ChenFZK19,DBLP:conf/uss/Tang0TZ21}.
An orthogonal line of research tries to detect whether a given input image contains a trigger, mostly by finding anomalies in activations or latent representations when propagating the input through the model at hand~\cite{DBLP:conf/aaai/ChenCBLELMS19,DBLP:conf/nips/Tran0M18,DBLP:conf/acsac/GaoXW0RN19}.

\par\smallskip\textbf{Hardware \Trojans.}
For a general overview of hardware \trojans, see \cite{DBLP:journals/iet-cdt/XueGLYO20,DBLP:journals/integration/LiLZ16,DBLP:journals/dt/TehranipoorK10a}.
The idea of hardware \trojans targeting neural networks was first proposed by Clements~\etal~\cite{DBLP:journals/corr/abs-1806-05768} and Li~\etal~\cite{DBLP:conf/isvlsi/LiYNWWWY18} in 2018.
Other works~\cite{DBLP:conf/ats/YeH018} require manipulations to the inputs to trigger the hardware \trojan which then bypasses the machine-learning accelerator altogether.
More recent \trojan attacks trigger on intermediate layer outputs~\cite{DBLP:journals/corr/abs-1911-00783}, are inserted into the on-chip memory controller~\cite{DBLP:journals/tcad/HuZDLZYLX21}, or target activation parameters~\cite{DBLP:journals/esl/MukherjeeC22}.
Neither of these works addresses the insertion of a machine-learning backdoor into a trained learning model during inference. 

Hardware acceleration for machine-learning is also susceptible to non-\trojan attacks.
Liu~\etal~\cite{DBLP:conf/dac/LiuCZL20} injected glitches for untargeted misclassification and demonstrated applicability using Xilinx Vitis AI.
Hong~\etal~\cite{DBLP:conf/uss/HongFKGD19} found that hardware attacks inducing a fault to a single parameter can often cause an accuracy drop of around 90\%.
Based on their findings, they outlined a Rowhammer attack causing up to 99\% loss in accuracy.
Caner~Tol~\etal~\cite{DBLP:conf/dsn/TolIASZ23} presented a backdoor attack, again using Rowhammer.
Finally, Alam \etal~\cite{DBLP:conf/fdtc/AlamTGTF19} investigated \ac{RAM} collisions caused by concurrent writes.

==> sections/XX_background.tex <==
\section{Technical Background}
\label{dpu_trojan::sec::background}

We start by introducing
%
technical background on the hardware design process and its use in machine-learning acceleration.

\subsection{Hardware Design Process}
\label{dpu_trojan::subsubsec::hardware_design}
\todo{not only discuss process, but also threats and weaknesses}
From a high-level perspective, we distinguish between hardware implemented either as an \ac{ASIC} or \ac{FPGA}. 
For \acp{ASIC}, the hardware is fixed after manufacturing; examples include \acsp{CPU}, \acsp{GPU}, memory chips, and cryptographic co-processors. 
In contrast, \acp{FPGA} can be reconfigured in-field to implement arbitrary user-defined functionality.  
This configuration is done using a \textit{bitstream} that is uploaded to the \ac{FPGA}.
In both cases, the development of the hardware is a complex multi-stage process, involving a plethora of stakeholders and supply chains, often crossing international borders. 

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.45\linewidth}
        \centering
        \includegraphics[width=0.7\linewidth]{figures/hw_design_process.pdf}
        \caption{Hardware Design Process}
        \label{dpu_trojan::subfig::hw_design_process}
    \end{subfigure}
    \hspace{0.04\linewidth}
    \begin{subfigure}{0.45\linewidth}
        \centering
        \includegraphics[width=0.7\linewidth]{figures/ml_design_process.pdf}
        \caption{Machine-Learning Pipeline}
        \label{dpu_trojan::subfig::ml_design_process}
    \end{subfigure}
    \caption{High-level overview of hardware design and manufacturing as well as machine learning training and inference.}
    \label{dpu_trojan::fig::design_flow}
\end{figure}

\autoref{dpu_trojan::subfig::hw_design_process} depicts the high-level hardware design process.
At first, hardware designs for both \acp{ASIC} and \acp{FPGA} are described in a \ac{HDL} such as Verilog or VHDL. 
These high-level languages represent the hardware's design and semantics independent of the manufacturing process. 
Next, the design is transformed into a \emph{gate-level netlist} composed of logic gates and their interconnections by a \textit{synthesizer}. 
The netlist is then implemented, that is, technology-mapped, placed, and routed. 
The required tools are provided by \ac{EDA} vendors (\eg,~Synopsys, Cadence, or Siemens) or \ac{FPGA} manufacturers (\eg,~Xilinx, Intel). 
The output is a \emph{technology-mapped netlist} comprising the gates available for the target \ac{ASIC} manufacturing process or the \ac{FPGA} architecture.
This netlist often takes the form of a GDSII layout for \ac{ASIC} manufacturing or a bitstream used to configure \acp{FPGA}.

Third-party hardware components, so called \emph{\ac{IP} cores}, can be integrated throughout the entire process. 
For instance, \ac{IP} cores provided as \ac{HDL} files may be added at design time.
Such third-party components are widely used for economic reasons, as they lower development time and cost. 
They implement a variety of functionality, ranging from cryptographic engines to machine-learning accelerators.
To prevent \ac{IP} disclosure and infringement, vendors often protect their cores using encryption, \eg, following standards like \acs{IEEE}~1735~\cite{Automation2015}. 
In the context of the paper at hand, we note that machine-learning accelerators undergo the same design process independent of whether they are implemented as \acp{ASIC} or \acp{FPGA}.


\subsection{Machine-Learning Acceleration}
\label{dpu_trojan::subsubsec::ml_acceleration}

Machine learning is rarely conducted on regular \acsp{CPU} anymore. 
Instead, specialized hardware accelerates expensive computations, such as tensor multiplications and convolutions, thereby significantly improving time and energy efficiency.
Such \emph{machine-learning accelerators} range from high-performance \acsp{GPU} for training, such as NVIDIA's A100 and H100, to versatile inference solutions, like Apple's neural processing unit, also suitable for embedded and mobile devices.

Technically, we can distinguish between hardware acceleration for training and inference. 
While the former is crucial for training complex and large neural networks, the latter is vital for the deployment of machine learning in real-time or resource-constrained applications, which often run on embedded (mobile) devices.
Our work focuses on inference as it allows an attacker to manipulate predictions of a deployed learning model from within modified hardware.

To apply hardware acceleration for inference, the learning model needs to be specifically prepared after training, as shown in \autoref{dpu_trojan::subfig::ml_design_process}. 
First, the model parameters are often quantized, \ie, their bit width is reduced and floating-point values are converted to fixed-point. 
This increases computing and memory efficiency, while maintaining the model's accuracy to the extent possible. 
Next, the quantized model is compiled into a representation suitable for execution on the accelerator, such as TensorFlow Lite by Google or the proprietary format used in Xilinx \acp{FPGA}. 

Note that the trained model is adapted to the hardware accelerator, but not vice versa.
Machine-learning accelerators are agnostic to the deployed models and their architecture.
In particular, a hardware \ac{IP} core accelerating tensor multiplications can be utilized for inference on various neural network architectures and layers. 
This versatility renders our attack challenging, as we need to determine the right execution context for activating the backdoor functionality.


